Infrared spectroscopic confirmation of z~2 photometrically-selected obscured quasars

The census of obscured quasar populations is incomplete, and remains a major unsolved problem, especially at higher redshifts, where we expect a greater density of galaxy formation and quasar activity. We present Gemini GNIRS near-infrared spectroscopy of 24 luminous obscured quasar candidates from the Sloan Digital Sky Survey's Stripe 82 region. The targets were photometrically selected using a WISE/W4 selection technique that is optimized to identify IR-bright and heavily-reddened/optically-obscured targets at $z>1$. We detect emission lines of ${\rm H\alpha}$, ${\rm H\beta}$, and/or ${\rm[ O~III]}$ in 23 sources allowing us to measure spectroscopic redshifts in the range $1<z<3$ with bolometric luminosities spanning $L=10^{46.3}-10^{47.3}$ erg s$^{-1}$. We observe broad $10^3-10^4$ km s$^{-1}$ Balmer emissions with large ${\rm H\alpha}/{\rm H\beta}$ ratios, and we directly observe a heavily reddened rest-frame optical continuum in several sources, suggesting high extinction ($A_V\sim7-20$ mag). Our observations demonstrate that such optical/infrared photometric selection successfully recovers high-redshift obscured quasars. The successful identification of previously undetected red, obscured high-redshift quasar candidates suggests that there are more obscured quasars yet to be discovered.

==> gnirs-appdix-v3.tex <==
\appendix 
\section{Source spectra}\label{apx:spectra}

\begin{figure*}
     \begin{tabular}{c}
     \begin{tabular}{cc}
	 \includegraphics[width=0.9\columnwidth]{spectra/J0213+0024_v2.png} &
	 \includegraphics[width=0.9\columnwidth]{spectra/J2243+0017_v2.png} 
	 \end{tabular}
        \\
    \begin{tabular}{ccc}
	 \includegraphics[width=0.31\textwidth]{spectra/J0149+0052_v2.png} &
	 \includegraphics[width=0.31\textwidth]{spectra/J0152-0024_v2.png} &
	 \includegraphics[width=0.31\textwidth]{spectra/J0215+0042_v2.png} \\
	 \includegraphics[width=0.31\textwidth]{spectra/J2259-0009_v2.png} &
      \includegraphics[width=0.31\textwidth]{spectra/J2334+0031_v2.png} & 
      \includegraphics[width=0.31\textwidth]{spectra/J0041-0029_v2.png} \\
	 \end{tabular}
	 \end{tabular}
	 \caption{\textcolor{red}{[placeholder]} `A' spectra with strong continuum and emission lines. Boxcar smoothed in thick black line.}
	 \label{fig:spect_show} 
\end{figure*}
